Scaling Hyperledger Fabric Using Pipelined Execution and Sparse Peers

Permissioned blockchains are becoming popular as data management systems in the enterprise setting. Compared to traditional distributed databases, blockchain platforms provide increased security guarantees but significantly lower performance. Further, these platforms are quite expensive to run for the low throughput they provide. The following are two ways to improve performance and reduce cost: (1) make the system utilize allocated resources efficiently; (2) allow rapid and dynamic scaling of allocated resources based on load. We explore both of these in this work. We first investigate the reasons for the poor performance and scalability of the dominant permissioned blockchain flavor called Execute-Order-Validate (EOV). We do this by studying the scaling characteristics of Hyperledger Fabric, a popular EOV platform, using vertical scaling and horizontal scaling. We find that the transaction throughput scales very poorly with these techniques. At least in the permissioned setting, the real bottleneck is transaction processing, not the consensus protocol. With vertical scaling, the allocated vCPUs go under-utilized. In contrast, with horizontal scaling, the allocated resources get wasted due to redundant work across nodes within an organization. To mitigate the above concerns, we first improve resource efficiency by (a) improving CPU utilization with a pipelined execution of validation & commit phases; (b) avoiding redundant work across nodes by introducing a new type of peer node called sparse peer that selectively commits transactions. We further propose a technique that enables the rapid scaling of resources. Our implementation - SmartFabric, built on top of Hyperledger Fabric demonstrates 3x higher throughput, 12-26x faster scale-up time, and provides Fabric's throughput at 50% to 87% lower cost.

==> implementation.tex <==
% \section{Implementation}
% \label{implementation}
% The overall implementation added 15k lines of golang code to Fabric v1.4 excluding test and generated code.
% The dependency graph was implemented using two queues: one for distributed transactions and another for
% a normal transactions. Each entry in the queue pointed to transactions blocking it. These pointers were
% used to track dependencies. The dirty state component was implemented using a trie in order to handle
% validation of range queries.
% The implementation of sparse peer itself was straightforward as it mostly involved making the code
% ignore transactions outside of the peer's filter. For modifying filters of a peer on the fly by
% the administrators, we implemented a system smart-contract that gave an interface to modifying the peer's filters.
%For splitting and merging of peers, we added a controller between the peers that handled requesting
%and sending "diffs" for stateDB and historyDB in a given \textit{start block number} and \textit{end block number}
% For responding to such requests, a controller would acquire a snapshot on the underlying levelDB instances.
% An alternative to this would be to query the ledger component using its range query API. However
% that would acquire a read lock on the instance, causing the commit process to halt till we 
% complete the copy operation. Using a levelDB snapshot frees us from this problem.


==> tables/scaling-quorum.tex <==
	\begin{table}
	\vspace{-.2cm}
		\small{
	\centering
	\caption{\small{Impact of scaling techniques on Quorum.}}
	\label{table:scalability-quorum}
	\begin{tabular} {| c | c | c | c |}%{  | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.6cm} |}
        \hline
        {\textit{workload}} &
        {\textit{\pbox{1.5cm}{maximum throughput}}} &
		{\textit{\pbox{1cm}{\#vCPUs}}} &
        {\textit{\pbox{1.8cm}{\#peers per organization}}} \\ \hline

        smallbank & 1790 & \multirow{2}{*}{1, 2, 4, 8, 16} & \multirow{2}{*}{1} \\ \cline{0-1}
		ycsb & 1000 & & \\ \hline
        smallbank & 1790 & \multirow{2}{*}{16} & \multirow{2}{*}{1, 2, 4} \\ \cline{0-1}
		ycsb & 1000 &  & \\ \hline
  \end{tabular}
	\vspace{-.2cm}
}
\end{table}


==> tables/scaling.tex <==
{
	\begin{table}
	\vspace{-.2cm}
		\small{
	\centering
	\caption{\small{Impact of scaling techniques on Fabric.}}
	\label{table:scalability}
	\begin{tabular} {| c | c | c | c |}%{  | p{1.2cm} | p{1.2cm} | p{1.2cm} | p{1.6cm} |}
        \hline
        {\textit{workload}} &
        {\textit{\pbox{1.5cm}{maximum throughput}}} &
		{\textit{\pbox{1cm}{\#vCPUs}}} &
        {\textit{\pbox{1.8cm}{\#peers per organization}}} \\ \hline

        smallbank & 1790 & \multirow{2}{*}{1, 2, 4, 8, 16} & \multirow{2}{*}{1} \\ \cline{0-1}
		ycsb & 1000 & & \\ \hline
        smallbank & 1790 & \multirow{2}{*}{16} & \multirow{2}{*}{1, 2, 4} \\ \cline{0-1}
		ycsb & 1000 &  & \\ \hline
		% channels & 1 & \multirow{2}{*}{1, 2, 4, 8} & &  & 3034 & limited data access \\ \cline{0-1}\cline{7-8}
		% peers and channels & 1, 4 & & &  & 9964 & absolute data silos \\ \cline{0-2}\cline{6-8}
		% simple endorsement & 1 & \multirow{2}{*}{1} & & & simple & 3120 & weaker trust \\ \cline{0-1} \cline{6-8}
		% \textbf{our approach} & 4 & & & & complex & \textbf{6328} & ---\\ \hline
		% \multicolumn{2}{c|}{same block} & among conflicts&\\ \hline
	% \CheckmarkBold & \CheckmarkBold & nearConflict & farConflict \\ \hline
	% \CheckmarkBold & \CheckmarkBold & farConflict & nearConflict \\ \hline
	% \CheckmarkBold & \XSolidBrush & nearConflict & farConflict \\ \hline
	% \XSolidBrush & \CheckmarkBold & farConflict & \multirow{3}{*}{nearConflict} \\ \cline{0-2}
	% \XSolidBrush & \XSolidBrush & - &  \\ \cline{0-2}
	% \XSolidBrush & none & - &  \\ \hline
	%1 & \multicolumn{2}{c|}{in the same block as T} & nearConflict \\ \hline
	%2 & \multicolumn{2}{c|}{not in same block} & nearConflict \\ \hline

  \end{tabular}
	\vspace{-.2cm}
}
\end{table}
}



==> tables/vmcosts.tex <==
{
      \begin{table}[]
      \begin{tabular}{lllllll}
            & AWS         &          & Google Cloud   &          & Azure    &          \\
      Cores & Instance    & Cost     & Instance       & Cost     & Instance & Cost     \\
      2     & m6g.large   & \$56.21  & e2-standard-2  & \$58.01  & B2MS     & \$60.74  \\
      4     & m6g.xlarge  & \$112.42 & e2-standard-4  & \$113.11 & B4MS     & \$121.18 \\
      8     & m6g.2xlarge & \$224.84 & e2-standard-8  & \$223.29 & B8MS     & \$243.09 \\
      16    & m6g.4xlarge & \$459.68 & e2-standard-16 & \$443.67 & B16MS    & \$486.18
      \end{tabular}
      \end{table}
}
